Projection-based significance test for longitudinally collected functional data under a crossover design

Wearable devices for continuous electronic health monitoring often capture data at frequent intervals under a dense functional design. The focal point is the analysis of longitudinal functional data, wherein functional trajectories are observed repeatedly over time. This work is motivated by the interest in assessing the efficacy of a noninflammatory medication, meloxicam, on the daily activity levels of household cats with a pre-existing condition of osteoarthritis under a crossover design. An accelerometer records these activity profiles at a minute level over the entire study period. To this aspect, we propose an orthogonal projection-based pseudo-generalized F test to determine the significance of the functional treatment effect under a functional additive crossover model while accounting for carryover effects and baseline covariates. Under mild conditions, we derive the asymptotic null distribution of the test statistic and the theoretical power function when the projection function is estimated from the data. Numerical studies demonstrate that the proposed test maintains size, proves powerful in detecting the smooth effect of meloxicam, and exhibits high efficiency compared to bootstrap-based alternatives. Application of the test on the accelerometric activity profiles reveals a strong positive effect of meloxicam on the joint pain score of the cats after adjusting for other baseline covariates.

==> supplement_labels.tex <==
% Section, equation, figure, table and assumption numbers of the
% Supplementary Material, which the manuscript refers to.
\makeatletter
\newlabel{sec: modelformulation}{{S1}{1}{Truncated polynomial basis formula for the projected model}{}{}}
\newlabel{sec: orthogonalbasis}{{S2}{2}{Selection of the orthogonal basis}{}{}}
\newlabel{sec: discussionofassump}{{S3}{2}{Discussion of assumptions}{}{}}
\newlabel{assump: chap3mibounded}{{1}{2}{Discussion of assumptions}{}{}}
\newlabel{assump: chap3epsiloncontinuous}{{2}{2}{Discussion of assumptions}{}{}}
\newlabel{assump: chap3normality}{{3}{2}{Discussion of assumptions}{}{}}
\newlabel{assump: chap3mineigenvalue}{{4}{2}{Discussion of assumptions}{}{}}
\newlabel{sec: additionalresults}{{S4}{3}{Additional results related to PROLIFIC}{}{}}
\newlabel{theorm: chap3trtwcarrynull}{{1}{3}{Additional results related to PROLIFIC}{}{}}
\newlabel{eqn: tau_alt}{{S.1}{3}{Additional results related to PROLIFIC}{}{}}
\newlabel{eqn: chap3asymptnullqpGFtrtwcarry}{{S.2}{3}{Additional results related to PROLIFIC}{}{}}
\newlabel{theorm: chap3trtwocarrynull}{{2}{4}{Additional results related to PROLIFIC}{}{}}
\newlabel{eqn: chap3asymptnullqpGFtrtwocarry}{{S.3}{4}{Additional results related to PROLIFIC}{}{}}
\newlabel{sec: modelestimation}{{S5}{4}{Details of estimation of FACM}{}{}}
\newlabel{sec: additionalsimresults}{{S6}{4}{Additional results relevant to the simulation study}{}{}}
\newlabel{tab: size_zc}{{T1}{5}{Empirical size of \textbf {\em Ad-ZC} based on 5000 simulations}{}{}}
\newlabel{sec: additionaldataresults}{{S7}{5}{Additional figures relevant to the meloxicam study}{}{}}
\newlabel{sec: proofs}{{S8}{5}{Proof of theorems and corollaries}{}{}}
\newlabel{fig: rawandrollact}{{F1}{6}{Daily raw activity profiles for a randomly selected cat (cat number $62$) over the days $4,8,10,12$, and $16$ in all the four periods}{}{}}
\newlabel{eqn: chap3GVG}{{S.4}{6}{Proof of theorems and corollaries}{}{}}
\newlabel{fig: logcumactid1-2}{{F2}{7}{Cumulative average of the log activity profiles from $5$AM to $10$PM for two randomly selected cats (cat number $10$ and $60$) over the days $4,8,10,12$, and $16$ in all the four periods. No activities were recorded for the cat number $10$ in the last period}{}{}}
\newlabel{fig: logcumactid3-4}{{F3}{8}{Cumulative average of the log activity profiles from $5$AM to $10$PM for two randomly selected cats (cat number $36$ and $39$) over the days $4,8,10,12$, and $16$ in all the four periods}{}{}}
\newlabel{fig: freqmipandboxplots}{{F4}{9}{(a) Frequency distribution of the number of PA profiles ($m_{ip}$) observed for each of the four periods. (b) Boxplot of the baseline age (in years) and weight (in lbs) of the cats}{}{}}
\newlabel{fig: chap3allbaselinecov}{{F5}{10}{(a) Estimated mean $\widehat {\mu }(\cdot ,Age)$ at six equidistant quantiles of the distribution of $Age$ in the data, (b) Estimated effect of weight, $\widehat {\beta }_1(s)$ (c) Estimated effect of weekend, $\widehat {\beta }_2(s)$ (d) Estimated effect of DJD score, $\widehat {\beta }_3(s)$. The numbers in the y-axis are multiplied by $100$}{}{}}
\newlabel{eqn: chap3relationWdelta}{{S.5}{11}{Proof of theorems and corollaries}{}{}}
\newlabel{eqn: chap3relationdeltadelta*}{{S.6}{11}{Proof of theorems and corollaries}{}{}}
\newlabel{eqn: chap3RSS0exp}{{S.7}{11}{Proof of theorems and corollaries}{}{}}
\newlabel{eqn: chap3RSS1exp1}{{S.8}{11}{Proof of theorems and corollaries}{}{}}
\newlabel{eqn: chap3Vinvexp}{{S.9}{12}{Proof of theorems and corollaries}{}{}}
\newlabel{eqn: chap3RSS1exp2}{{S.10}{12}{Proof of theorems and corollaries}{}{}}
\newlabel{eqn: chap3RSS0expindelta}{{S.11}{12}{Proof of theorems and corollaries}{}{}}
\newlabel{eqn: chap3RSS1expindelta}{{S.12}{12}{Proof of theorems and corollaries}{}{}}
\newlabel{eqn: chap3R0-R1Expr}{{S.15}{13}{Proof of theorems and corollaries}{}{}}
\newlabel{eqn: chap3R1Expr}{{S.16}{13}{Proof of theorems and corollaries}{}{}}
\makeatother

